Hybrid Reinforcement Learning from Offline Observation Alone

We consider the hybrid reinforcement learning setting where the agent has access to both offline data and online interactive access. While Reinforcement Learning (RL) research typically assumes offline data contains complete action, reward and transition information, datasets with only state information (also known as observation-only datasets) are more general, abundant and practical. This motivates our study of the hybrid RL with observation-only offline dataset framework. While the task of competing with the best policy "covered" by the offline data can be solved if a reset model of the environment is provided (i.e., one that can be reset to any state), we show evidence of hardness when only given the weaker trace model (i.e., one can only reset to the initial states and must produce full traces through the environment), without further assumption of admissibility of the offline data. Under the admissibility assumptions -- that the offline data could actually be produced by the policy class we consider -- we propose the first algorithm in the trace model setting that provably matches the performance of algorithms that leverage a reset model. We also perform proof-of-concept experiments that suggest the effectiveness of our algorithm in practice.

==> main.tex <==
% \documentclass{article}
% \usepackage{amsthm,mkolar_definitions,color,comment}
% \usepackage{algorithmicx}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}

% \usepackage{natbib}
% \bibliographystyle{plainnat}

% \bibpunct{(}{)}{;}{a}{,}{,}

% \usepackage[dvipsnames]{xcolor}


% \usepackage[colorlinks]{hyperref}
% \hypersetup{
%     citecolor=[RGB]{50,100,170},
%     linkcolor=[RGB]{50,100,170},
%     urlcolor=[RGB]{255,102,178}}

% \usepackage{fancyref}


% \usepackage[left=2cm,top=2cm,right=2cm]{geometry}

% \usepackage{graphicx}
% \usepackage{comment}
% \usepackage{color-edits}
% \usepackage{showlabels}
% \usepackage{xspace}
% \usepackage{nicefrac}
% \usepackage{booktabs}


% \usepackage{transparent}
% \newcommand{\algcommentlight}[1]{\textcolor{blue!70!black}{\transparent{0.5}\small{\texttt{\textbf{//\hspace{2pt}#1}}}}}
% \newcommand{\algcomment}[1]{\textcolor{blue!70!black}{\footnotesize{\texttt{\textbf{//
%           #1}}}}}
% \newcommand{\algcommentbig}[1]{\textcolor{blue!70!black}{\footnotesize{\texttt{\textbf{/*
%           #1~*/}}}}}

% \algrenewcommand\algorithmicrequire{\textbf{require}}


% \addauthor{ak}{red}

% %\usepackage{color}
% \newcount\Comments  % 0 suppresses notes to selves in text
% \Comments=1 % TODO: change to 0 for final version
% \definecolor{darkgreen}{rgb}{0,0.5,0}
% \definecolor{darkred}{rgb}{0.7,0,0}
% \definecolor{teal}{rgb}{0.3,0.8,0.8}
% \newcommand{\kibitz}[2]{\ifnum\Comments=1\textcolor{#1}{#2}\fi}
% \newcommand{\yuda}[1]{\kibitz{cyan}{[YS: #1]}}
% \newcommand{\jab}[1]{\kibitz{darkred}{[JAB: #1]}}


% \usepackage{color-edits}

% \newcommand{\rank}{\mathsf{rank}}
% \newcommand{\tv}{\mathsf{TV}}
% \newcommand{\zoom}{d_{\textup{zoom}}}
% \newcommand{\disc}[1]{\textsf{disc}_{#1}}
% \newcommand{\reg}{\mathsf{Reg}}
% \newcommand{\ccov}{C_\mathsf{cov}}
% \newcommand{\Mreset}{\Mcal_\mathsf{reset}}
% \newcommand{\pif}{\pi^\mathsf{f}}
% \newcommand{\pib}{\pi^\mathsf{b}}
% \newcommand{\IPM}{\mathsf{IPM}}
% \newcommand{\piunif}{\pi^\mathsf{unif}}
% \newcommand{\Psdp}{\textsc{Psdp}} 
% \newcommand{\piin}{\pi^\mathsf{in}} 
% \newcommand{\Fail}{\textsc{Fail}} 
% \newcommand{\Foobar}{\textsc{Foobar}} 
% \newcommand{\epsminmax}{\epsilon^\textsf{mm}} 
% \newcommand{\epsforward}{\epsilon^\textsf{for}} 
% \newcommand{\epsback}{\epsilon^\textsf{back}} 
% \newcommand{\hyrlo}{\textsc{HyRLO}}
% \newcommand{\ilfo}{\textsc{ILfO}}

% \begin{document}

% \title{Hybrid Reinforcement Learning from Offline Observation Alone}
% \maketitle

% \begin{abstract}
    
% \end{abstract}

% \section{Introduction}

% Recently, explosive growth in the availability of offline data for interactive decision making problems \citep{dasari2019robonet,qin2022neorl,mathieu2023alphastar,padalkar2023open} and the general access to interact with the environment for feedback \jab{What does that mean} led to the development of Hybrid Reinforcement Learning (Hybrid RL) \citep{ross2012agnostic,song2022hybrid}. This paradigm blends the exploratory strengths of offline data with the dynamism of online interaction, creating a new learning environment towards more efficient solutions that are robust against the issues of verifiability and compounding errors \citep{song2022hybrid, wagenmaker2023leveraging,nakamoto2023cal}.  \jab{This sounds fancy, but I'm not sure whatit's really saying}. Traditionally, RL has oscillated between purely offline and online realms, each with its inherent challenges. Offline learning, while data-rich, often lacks the adaptability of real-world scenarios due to its instability \citep{wang2021instabilities}. Conversely, online learning offers real-time data but at the cost of increased complexity due to the requirement of exploration, both statistically and computationally \citep{du2019good, kane2022computational}. Recognizing these limitations, Hybrid RL demonstrated the synergistic benefits it offers. Earlier studies in this domain have predominantly utilized extensive offline datasets, encompassing state, action, reward, and subsequent state information. This comprehensive data approach has proven beneficial, highlighting the statistical and computational superiority of Hybrid RL over its singular counterparts \citep{song2022hybrid,hu2023reboot}.

% However, a critical observation emerges: the necessity for expansive datasets in such a rich format poses a significant barrier. In practice, most large scale dataset exists in the format of videos \cite{grauman2022ego4d,grauman2023ego} (imagine using video demonstations from Youtube). In addition, the requirement of the existence of actions in the dataset is restrictive because actions do not generalize between different modalities: one should not expect to use human actions for robot actuators, and different robots have different action spaces as well. The current solution of collecting different actions for different modalities is both tedious and not salable. Another issue of classic offline dataset format is that, in practice, a reward function is not always known, which sometimes requires additional effort in reward shaping. However, in reality, even deliberately designed reward function may end up as being sub-optimal for policy optimization \citep{ma2023eureka}. 

% In this work, we initiate the study of the setting of Hybrid RL from Observation Alone (\hyrlo). We focus on the simplest setting where the offline data only contains (not necessarily consecutive) state data. Previous there has been a rich line of studies on the different formats of offline dataset in different interactive decision making problems \citep{abbeel2004apprenticeship, ziebart2008maximum, torabi2018generative,sun2019provably,ma2022versatile,li2023mahalo}, the rigorous formulation of the \hyrlo{} setting is still absent. We believe the study of \hyrlo{} fillis in the last missing piece of all possible settings in Hybrid RL, offline RL and Imitation Learning, with respect to the different combinatorics of state, action, reward, next-state in the offline dataset. 

% As a general and powerful learning paradigm, the \hyrlo{} has indeed been attracting adequate attention. Previous studies that fell into the \hyrlo{} setting can be mostly characterized as two ways: the first one is to leverage the offline state data to perform representation learning (i.e., require a separate pretraining stage) \citep{nair2018visual,ma2022vip,ghosh2023reinforcement}, and then to use the learned feature map to speed up the downstream online RL training. However, the state-only offline dataset, although less informative than the canonical offline data, still provide rich signcal towards decision-making. In this work, we will show that we can indeed directly use the offline state data for decision-making. The second way is to rely on a reset model (or assume an exploratory reset distribution) \citep{ kakade2002approximately,bagnell2003policy}, which only holds true if a simulator is available and thus is not the most practical scenario to consider. In this work, we show that we can solve the \hyrlo{} problem without the reset model (i.e., with the trace model which only resets at the initial step), and in fact reduce to the reset model setting with the practical assumption of admissibility of the offline data.

% \subsection{Contributions}
% We initiate the theoretical study of the \hyrlo{} setting, and provide the first provably algorithm for this setting. Specifically:
% \begin{itemize}
%     \item \textbf{Mathematical formulation.} We provide the first theoretical formulation of the \hyrlo{} in the most general terms, where the offline dataset only contains states that are not necessarily consecutive (i.e., from the same trajectories). 
%     \item \textbf{Separations between reset model and trace model.} Given the \hyrlo{} setting is solved when a reset model is available \citep{bagnell2003policy}, we show a reduction to the trace model to reset model setting via the admissibility condition, where the offline distribution is realizable by the policy class. In addition, we demonstrate exponential separations in sample complexities between trace and reset models if the admissibility condition is violated. 
%     \item \textbf{Efficient algorithm.} We provide the first provable solution to the \hyrlo{} setting, FOrward Observation-matching BAckward Reinforcement Learning (\Foobar). With admissibility, \Foobar{} requires the same order of samples as the previous reset model algorithm \citep{bagnell2003policy}, to compare with the best policy covered by the offline distribution.
%     \item \textbf{Empirical evaluation.} We perform experiments to show the effectiveness of our algorithm on two challenging benchmarks: the rich-observation combination lock \citep{misra2020kinematic} and high-dimensional robotics manipulation tasks \citep{rajeswaran2017learning}. We compare with the state-of-the-art algorithms in the canonical hybrid RL setting, and investigate the gap due to the missing information in the offline dataset. 
% \end{itemize}

% \section{Related Work}
% \paragraph{Hybrid RL.} Hybrid RL defines the setting where the agent has access to both offline data (usually generated by policies with a mixture of qualities) \citep{levine2020offline} and online interaction access. This learning framework has recently gained increasing interest due to its potential for efficient learning and practical values \citep{ross2012agnostic,nair2020awac,xie2021policy,song2022hybrid,lee2022offline,niu2022trust,ball2023efficient,nakamoto2023cal,wagenmaker2023leveraging,li2023reward,zhang2023policy,zhou2023offline}. Previous works follow the standard offline RL setting where the offline dataset contains the state, action, reward and next state information, and they have shown the statistical and computational benefit of the hybrid setting over pure online or offline setting. In this work, we consider a more general and challenging setting where the offline dataset only contains the state information. Many previous works have also considered this setting \citep{machado2017eigenoption,nair2018visual,schmeckpeper2020reinforcement,ma2022vip,baker2022video,seo2022reinforcement,ghosh2023reinforcement}, but the offline states are only used for representation learning in the separate pertaining stage, not RL. In addition, most of the works assume that the offline data consists of the state and next state pair, or states from trajectories. Our work conducts the first theoretical study in this setting and the proposed algorithm uses the offline data for RL directly, and we allow the state from each timestep to be generated from independent distributions.

% \paragraph{Learning from observation alone.} Prior to the \hyrlo{} setting, the learning from observation alone setting has also been considered in other interactive decision-making literature, such as imitation learning and offline reinforcement learning. In the imitation from observation alone setting (\ilfo) \citep{nair2017combining,torabi2018generative,sun2019provably,smith2019avid,song2020provably,zhu2020off,radosavovic2021state}, different from the traditional imitation learning setting where the expert dataset contains both state and action information, \ilfo{} assumes the dataset only contains the state information. Like \hyrlo{}, \ilfo{} also assume that the agent has the online interactive access with the environment. If one does not the online access, the offline counterpart is the offline imitation learning setting, where the agent has access to an offline dataset that contains only state information, but in addition, has access to a dataset of expert state. \citep{kim2021demodice,ma2022versatile,yu2023offline,pirotta2023fast}. However, all these settings require access to some labeled expert data, while our setting only requires a mixture quality of offline data that implicitly covers the optimal policy's trajectory. Towards a framework of more general settings, recently \citet{li2023mahalo} considers the offline setting with either missing reward or action information, two novel settings where previous theoretical studies were lacking.

% \paragraph{RL with reset model.} In the reset model setting, one assumes a sampling oracle that samples a next state according to the ground truth transition kernel, given a state-action pair. With a reset model, the \hyrlo{} problem can be solved by the well-known Policy Search by Dynamic Programming (\Psdp) algorithm {\citet{bagnell2003policy,uchendu2023jump}. \yuda{Should I do this? Or should I mention jsrl separately?} The reset model has been shown to have other favorable properties that contribute to overcoming statistical hardness in the general trace model setting \citep{amortila2022few,weisz2021query}. On the empirical side, \citet{sharma2022state} shows that if expert data is available, one can learn to reset by training a policy that brings that current policy to the expert state distribution after the rollout. Finally, under many situations, the access to a reset model is equivalent to the access to an exploratory reset distribution, which is sufficient for many classical efficient algorithms such as Conservative Policy Iteration \citep{kakade2002approximately} and Natural Policy Gradient \citep{kakade2001natural,agarwal2020optimality}.  

% \section{Preliminaries}
% We consider finite horizon MDPs $\Mcal = \{\Scal, \Acal, H, R, P\}$, where $H$ is the horizon, $\Scal$ is the state space, $\Acal$ is the action space, $R = \{R_h: \Scal \times \Acal \to [0,1]\}_{h=1}^H$ is the reward function, and $P = \{P_h: \Scal \times \Acal \to \Delta(\Scal)\}_{h=1}^H$ is the transition function, with the contention that $P_0(\emptyset)$ is the initial state distribution. We assume that the trajectory returns are bounded by $H$. Given a (potentially unstationary) policy $\pi \in \Pi = \{\Scal \to \Delta(\Acal)\}_{h=1}^H$, define the Q function of $\pi$ as $Q_h^\pi(s_h,a_h) = \EE_{\pi,P} \sum_{\tau=h}^H R_\tau(s_\tau,a_\tau)$, and we define the optimal policy as $\pi^\ast$. We define the function class to estimate the Q function as $\Fcal: \Scal \times \Acal \to [0,H]$. We also follow the conventional notation $d^\pi_h$ to denote either the state (or state-action) occupancy measure of $\pi$ at horizon $h$. 

% We study the hybrid RL setting \citep{song2022hybrid}, where the agent has online interaction access to the environment, and in addition, has offline data set $\{\Dcal_h\}_{h=1}^H$.  In the canonical hybrid RL setting, each dataset $\Dcal_h$ contains tuples $\{s^i_h,a^i_h,r^i_h,s^i_{h+1}\}_{i=1}^N$, where $N$ is the size of the offline dataset. The data in $\Dcal_h$ is drawn from some distribution $\mu_h$, i.e., $s^i,a^i \sim \nu_h$: for example, $\nu_h$ can be some visitation distribution of some policy $\pi$, and $r^i_h = R_h(s^i_h,a^i_h)$, and $s^i_{h+1} \sim P_h(\cdot \mid s^i_h, a^i_h)$. Here we consider the \hyrlo{} setting, where in the offline dataset we only have the single-timestep state data. That is, the offline dataset has the form $\Dcal_h = \{s^i_h\}_{i=1}^N$, where $s_h \sim \mu_h$, and $\mu_h$ is some distribution over the states at timestep $h$. 

% For the coverage notation, we mainly consider the density ratio coverage for simplicity: given any policy $\pi$, we define the density ratio coverage as
% $\ccov(\pi) = \min_{h \in [H]} \min_{s \in \Scal_h} \frac{d^\pi_h(s)}{\mu_h(s)}$.

% To measure the difference between distributions, we define the Integral Probability Metric ($\IPM$) \citep{muller1997integral} distance between two distributions $P$ and $Q$:
% \begin{align*}
%     \IPM_{\Gcal}(P,Q) = \sup_{g \in \Gcal} \left| \int g~dP - \int g~dQ \right|,
% \end{align*}
% which is defined by the test function class $\Gcal$. For example, when $\Gcal$ is all bounded functions, then it recovers TV distance. When $\Gcal$ is the set of all $L$-Lipschitz functions, then it recovers the Wasserstein distance.

% We make the difference between the two types of MDPs: we will denote the canonical trace MDPs as we defined above as $\Mcal$, where one can only reset at the initial state $P_0$. We also consider MPDs with the ability to reset: at any horizon $h$, for any $s_h \in \Scal_h$, and any action $a \in \Acal$, we can query $P_h$ and get a sample $s_{h+1} \sim P_h(\cdot \mid s_h,a_h)$. We denote this reset model $\Mreset$.                                                                 

% Finally, For a more streamlined representation, we introduce the concept of a partial policy which operates over a sequential segment of time steps, specifically $\sbr{l \dots r} \in [H]$. This is represented as $\Pi_{l:r} := \cbr{\pi : \bigcup_{h=l}^r \Scal \to \Delta(\Acal)}$. Given any two intervals $1 \leq t \leq h \leq H$, we consider two partial policies: $\pi \in \Pi_{1:t-1}$ and $\pi' \in \Pi_{t:h}$. The composition $\pi \circ_t \pi'$ represents a policy that follows $\pi$ for the initial $t-1$ steps and switches to $\pi'$ for the subsequent $h-t+1$ steps. Formally, this is defined as $(\pi \circ_t \pi')(s_l) = \pi(s_l)$ when $l < t$ and $(\pi \circ_t \pi')(s_l) = \pi'(s_l)$ for $t \leq l \leq h$. The notation $s_h \sim \pi$ implies that the state $s_h$ is selected according to the distribution defined by the law of $\pi$ and $P$, and we extend this notation to include the action $a_h$ as well, denoted as $s_h, a_h \sim \pi$. 

% \section{Algorithm}

% To see how to solve the hybrid RL with observation alone problem, in this section we first see how this problem is solved in the reset model setting. Then we will use a technique used in the \ilfo{} setting to reduce the trace model setting to the reset model setting. The resulting algorithm thus will be a two-phase algorithm: in the first phase, we run a careful reduction to the reset model setting, and in the second phase, we run the reset model algorithm to find the optimal policy. A high-level illustration of the algorithm is shown in \pref{fig:foobar}.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/foobar.pdf}
%     \caption{The forward and backward algorithm.}
%     \label{fig:foobar}
% \end{figure}

% \subsection{Backward Algorithm: PSDP}
% Suppose we have the reset model $\Mreset$, then as we mentioned hinted above, we can solve the \hyrlo{} problem with an existing algorithm: Policy Search by Dynamic Programming (\Psdp) \citep{bagnell2003policy}.
% The \Psdp{} algorithm proceeds in a backward fashion: from the last timestep $H$ to the first timestep $1$, at each time step $h$, the algorithm first samples states from the offline dataset: $s_h \sim \mu_h$. Then the algorithm samples random action $a_h \sim \piunif$, resets the model to $s_h,a_h$, and then sample $s_{h+1} \sim P_h(s_h,a_h)$. From $s_{h+1}$ the algorithm will roll out $s_{h+1}, a_{h+1}, \ldots, s_{H},a_{H} \sim \pi_{h+1}, \ldots, \pi_H$ (which are already learned in the previous iteration). Now we have samples of the return information $\sum_{\tau=h}^H R(s_\tau,a_\tau)$ for each $s_h,a_h$ we can use cost-sensitive classification to find the one-step optimal policy $\pi_h$ which maximizes the returns following $\pi_{h+1}, \dots, \pi_H$, the previous one-step optimal policies. Here we provide a value-based version of the \Psdp{} algorithm in \pref{alg:psdp}.

% \begin{algorithm}[t]
%     \caption{Policy Search by Dynamic Programming (\Psdp)}
%     \begin{algorithmic}[1]
%     \Require Offline dataset $\Dcal_h$, online sample size $N$.
%     \For{$h=H, \ldots, 1$}
%         \For{$n = 1, \ldots, N$}
%             \State Sample $s^n_h \sim D_h, a^n_h \sim \piunif$.
%             \State Reset $\Mreset$ to $s^n_h,a^n_h$ and sample $s^n_{h+1} \sim P_h(s^n_h,a^n_h)$.
%             \State Follow $\pi_{h+1:H}$ and get sample $r^n_{h:H} \sim \pi_{h+1:H}.$
%         \EndFor
%     \State Train regressor $f_h(s_h,a_h)$ on $r_{h:H}$: \algcommentlight{Estimate Q function.}
%         \begin{align*}
%             f_h = \argmin_{f \in \Fcal} \sum_{n=1}^N \left(f(s_h^{n},a_h^{n}) - \sum_{\tau=h}^H r_{\tau}^{n}\right)^2.
%         \end{align*}
%     \State Get one-step greedy policy $\pi_h(s_h) = \argmax_{a_h} f_h(s_h,a_h)$.
%     \EndFor
% \Return{Non-stationary backward policy $\pi_{1:H}$.}
%     \end{algorithmic}
%     \label{alg:psdp}
% \end{algorithm}

% Now with \Psdp, as long as the offline distribution $\mu$ that generates the offline dataset $\Dcal$ covers the optimal policy's trajectory (for example, the density ratio coverage $\ccov$ is finite), we will guarantee that the returned policy is close to optimal once the size of the offline and online dataset is large enough, as we will show in \pref{sec:analysis}.

% \subsection{Trace to Reset}

% However, in the \hyrlo{} setting, we do not have the reset model $\Mreset$ but the canonical trace model $\Mcal$. What can we do in this case? It turns out that with the help of the offline dataset, we can learn a policy $\pif$ that induces a close state distribution as $\mu$. Then suppose that for each timestep $h$, we have that $\|d^\pi_h - \mu_h\|$ is small, where $\|\cdot\|$ is some distance metric that we care about. Now if we want to reset to $s_h \sim \mu_h$, we can instead roll in the policy $\pi$ to timestep $h$, and we will get samples $s_h \sim \pi_h$ (as if we are sampling $s_h \sim \mu_h$), and then we can proceed to run \Psdp. Thus we have a reduction from the reset model setting to the trace model settting. The new algorithm is summarized in \pref{alg:psdp_trace}. Note the the only change is in line 4. We remark that similar ideas of using \Psdp{} with some roll in policy has also been explored in previous works \cite{mhammedi2023efficient,mhammedi2023representation}, where the roll in policy is trained from reward-free exploration techniques.

% \begin{algorithm}[t]
%     \caption{Policy Search by Dynamic Programming (\Psdp) with trace model}
%     \begin{algorithmic}[1]
%         \Require Roll in policy $\piin$, online sample size $N$.
%         \For{$h=H, \ldots, 1$}
%             \For{n = $1, \ldots, N$}
%                 \State Sample $s^n_h \sim \piin_{1:h}, a^n_h \sim \piunif$.
%                 \State Reset $\Mreset$ to $s^n_h,a^n_h$ and sample $s^i_{h+1} \sim P_h(s^n_h,a^n_h)$.
%                 \State Follow $\pi_{h+1:H}$ and get sample $r^n_{h:H} \sim \pi_{h+1:H}.$
%             \EndFor
%         \State Train regressor $f_h(s_h,a_h)$ on $r_{h:H}$: \algcommentlight{Estimate Q function}
%             \begin{align*}
%                 f_h = \argmin_{f \in \Fcal} \sum_{n=1}^N \left(f(s_h^{n},a_h^{n}) - \sum_{\tau=h}^H r_{\tau}^{n}\right)^2.
%             \end{align*}
%         \State Get one-step greedy policy $\pi_h(s_h) = \argmax_{a_h} f_h(s_h,a_h)$.
%         \EndFor
%     \Return{Non-stationary backward policy $\pi_{1:H}$.}
%     \end{algorithmic}
%     \label{alg:psdp_trace}
% \end{algorithm}

% \subsection{Forward Algorithm: FAIL}
% Now the only problem remains to learn a policy $\piin$ that induces a close state distribution as $\mu$. Inspired by the idea of state-moment-matching that prevails in \ilfo{} literature, we can adapt one of such algorithms, Forward Adversarial Imitation Learning (\Fail) \citep{sun2019provably}. \Fail{} learns a sequence of policy $\pi_{1:H}$ from $h=1$ to $H$ in a forward way. At each timestep $h$, \Fail{} rolls in the previous policies $\pi_{1:h-1}$ and sample $s_{h-1} \sim \pi_{1:h-1}$. Then we take a random action $a_{h-1} \sim \piunif$ and sample $s_{h} \sim P_h(\cdot \mid s_{h-1},a_{h-1})$. With the dataset $\{s_{h-1},a_{h-1},s_h\}$, we want to solve the following minmax game by finding a one-step policy $\pi_h$ such that we can minimize the $\IPM$ between $\pi_{1:h}$ and $\mu_{h}$, from which we have the sample $\Dcal_{h}$:
% \begin{align*}
%     \min_{\pi_h \in \Pi_h} \max_{g \in \Gcal_h} \sbr{\EE_{s_h \sim \pi_{1:h}} g(s_h) - \EE_{s_h \sim \mu_h} g(s_{h})},
% \end{align*}
% which can be estimated by the dataset collected online at time step $h$:
% \begin{align*}
%     \min_{\pi_h \in \Pi} \max_{g \in \Gcal_h} \underbrace{\left(\frac{1}{N} \sum_{n=1}^N \frac{\pi_h(a_{h-1}^{n} \mid s_{h-1}^{n})}{1/A} g(s_{h}^{n}) - \frac{1}{N'} \sum_{n=1}^{N'} g(s_{h}^{n})\right)}_{u(\pi_h, g)}.
% \end{align*}
% To solve the minmax game, we can use the typical best response vs. no-regret algorithm. We show one way to solve this minmax game in \pref{alg:minmax}. Note that line 3 could be solved with a linear programming oracle, and line 5 could be solved with a regularized cost-sensitive classification oracle \citep{sun2019provably}. 
% \begin{algorithm}[t]
%     \caption{Min-Max Game}
%     \begin{algorithmic}[1]
%     \Require Policy class $\Pi$, discriminator class $\Gcal$, number of iterations $T$, online dataset $\Dcal^{\mathsf{on}}$, offline dataset $\Dcal^{\mathsf{off}}$.
%     \State Randomly initialize $\pi_0 \in \Pi$.
%     \For{$t=1$ to $T$}
%     \State $g^t = \argmax_{g \in \Gcal} u(\pi^t, g).$\algcommentlight{LP Oracle.}
%     \State $u^t := u(\pi^t, g^t)$.
%     \State $\pi^{t+1} = \argmin_{\pi \in \Pi} \sum_{\tau=1}^t u(\pi, g^t) + \phi(\pi)$. \algcommentlight{Regularized CS Oracle.}
%     \EndFor
% \Return $\pi^{t^\ast}$ with $t^\ast = \argmin_{t \in [T]} u^t.$
%     \end{algorithmic}
%     \label{alg:minmax}
% \end{algorithm}

% Now we can see the \Fail{} algorithm iteratively finds the solution of the minmax problem in a forward way. We present the pseudocode of \Fail{} in \pref{alg:fail}.

% \begin{algorithm}[t]
% \caption{\Fail}
% \begin{algorithmic}[1]
% \Require Offline dataset $\{\Dcal^{\textsf{off}}_h\}$, value function class $\Gcal$, policy class $\Pi$, number of online samples N, number of iterations of minmax game $T$.
%     \For{$h=1$ to $H$}    
%     \State $\Dcal^{\textsf{on}}_h \leftarrow \emptyset$.
%     \For{$n=1, \ldots, N$}
%     \State Sample $s^n_{h-1}, a^n_{h-1}, s^n_{h} \sim \pi \circ_h \piunif$.
%     \State Add $(s^n_{h-1}, a^n_{h-1}, s^n_{h})$ to $\Dcal^{\textsf{on}}_h$.
%     \EndFor
%     % \State Define the discriminator class $\Gcal_h$:
%     % \begin{align*}
%     %     \Gcal_h = \cbr{\max_a \abr{f(\cdot,a) - f'(\cdot,a)} + \abr{f(\cdot,a^\ast) - f'(\cdot,a^\ast)} : f,f' \in \Fcal_h, a^\ast = \argmax_{a} f(\cdot, a)}.
%     % \end{align*}
%     \State Get $\pi_h$ from the return of \pref{alg:minmax} with inputs $\cbr{\Pi_h, \Gcal_h, T, \Dcal^{\textsf{on}}_h,\Dcal^{\textsf{off}}_h}$.
%     \EndFor
% \Return{$\pi_{1:H}$.}
%     \end{algorithmic}
%     \label{alg:fail}
% \end{algorithm}

% \subsection{Forward-backward Algorithm: FOOBAR} Now we are ready to present the proposed algorithm, FOward Observation-matching BAckward Reinforcement learning (\Foobar). We present the pseudocode in \pref{alg:foobar}. In the foward phase, we run \Fail{} that outputs a sequence of policies $\pif_{1:H}$ whose state visitation distribution is close to the offline distribution $\mu$. However, one needs to be very careful here because we have never defined the discriminator class we will use for the forward run. It turns out that selecting an arbitrary discriminator class will result in a polynomial dependency on the number of states (see Theorem 3.2 of \citet{sun2019provably}), which is unfavorable given the fact that we already have an offline state dataset to imitate so such dependency should be avoidable in the case with a relatively high-quality offline dataset (e.g., not a uniform distribution over states). Indeed a polynomial dependency on the state is avoidable by a careful construction of the discriminator class based on the value function class that we use in the backward pass (\pref{eq:discriminator}). We provide the justification of such construction in \pref{app:proof_foobar}. Then in the backward phase, we run \Psdp-trace with the rollin policy $\piin = \pif_{1:H}$, and get the refined policies $\pib_{1:H}$, which will be close to optimal if $\mu$ covers the optimal policy's trajectory. 

% \begin{algorithm}[t]
%     \caption{FOward Observation-matching BAckward Reinforcement learning (\Foobar)}
%     \begin{algorithmic}[1]
%     \Require Offline dataset $\Dcal^{\textsf{off}}$, value function class $\Fcal$, policy class $\Pi$.
%     \State Define the discriminator class $\Gcal_h$:  \algcommentlight{Discriminators take state as input while value functions take state-action as input.}
%     \begin{equation}\label{eq:discriminator}
%         \Gcal_h = \cbr{\max_a \abr{f(\cdot,a) - f'(\cdot,a)} + \abr{f(\cdot,a^\ast) - f'(\cdot,a^\ast)} : f,f' \in \Fcal_h, a^\ast = \argmax_{a} f(\cdot, a)}.
%     \end{equation}
%     \State $\pif_{1:H} \leftarrow$ \pref{alg:fail} with input $\cbr{\Dcal^{\textsf{off}}, \Gcal, \Pi}$.
%     \State $\pib_{1:H} \leftarrow$ \pref{alg:psdp_trace} with input $\cbr{\pif_{1:H}, \Fcal}$.
%     \end{algorithmic}
%     \label{alg:foobar}
% \end{algorithm}

% \section{Analysis}\label{sec:analysis}
% In this section we provide the analysis of the proposed algorithm. We will first show the performance guarantee of the forward algorithm, which determines the performance guarantee of the backward algorithm. We will start with the assumptions. The first assumption is on the property of the offline distribution. Note that all distributions mentioned in the following section denote the state marginal distribution. 

% \subsection{Admissibility}

% \begin{assumption}[Admissibility] \label{assum:admissibility}
%     We assume the offline distribution $\mu$ is admissible: $$\exists \pi \in \Pi, \forall h \in [H], \nbr{\mu_h - \pi_{1:h}}_{TV} = 0.$$
% \end{assumption}

% \begin{remark}
% \pref{assum:admissibility} captures the situations where the offline policy is generated by a single policy, stitching policies (due to non-stationarity) and a mixture of policies (proved in \pref{prop:mixture}), which is mostly how the offline dataset is generated in practice. The most practical way to break the assumption is with a simulator, and reset the simulator with a distribution that contradicts the dynamics of the MDPs, but this is not a very realistic scenario.
% \end{remark}

% In fact, we can also show that if \pref{assum:admissibility} breaks, then the problem is inherently hard. Next We show two hardness results when \pref{assum:admissibility} fails:

% \begin{proposition} \label{prop:hard_data}
%     There exists an MDP $\Mcal$ with deterministic transition and a set of offline datasets $\{\Dcal\}$, with arbitrary sample size $\abr{\Dcal} = N \geq 2$, collected from the inadmissible offline distribution $\mu$ with constant coverage: $\nbr{\frac{d^{\pi^\ast}}{\mu}}_{\infty} = 2$. Then for any algorithms $\textsf{Alg}$, denote the dataset collected by $\textsf{Alg}$ as $D_{\textsf{Alg}}$. Then unless $\abr{D_{\textsf{Alg}}} = \Omega(A^H)$,
%     denoting $\hat D$ as the empirical distribution of 
%     a dataset $D$, we have that
%     \begin{align*}
%         \min_{\Dcal} \nbr{\hat D_{\textsf{Alg}} - \hat \Dcal}_{TV} \geq 1.
%     \end{align*}
%     However, there exists an algorithm $\textsf{Alg}^{\textsf{reset}}$ that uses the offline dataset $\Dcal$ and reset model $\Mcal^{\textsf{reset}}$ that returns optimal policy $\pi^\ast$ with sample complexity $O(A)$.
% \end{proposition}

% The above statement is about the hardness on collecting a dataset that matches the offline dataset: when admissibility assumption is violated, in the worst case we need to collect a dataset that is exponentially large in the horizon; otherwise we do not even witness half of the data in the offline dataset. In the next proposition, we show another hardness result that has direct implications on the performance of the learned policy.

% \begin{proposition} \label{prop:hard_tv}
%     There exists MDP $\Mcal$ and inadmissible offline distribution $\mu$, such that $\nbr{\frac{d^{\pi^\ast}}{\mu}}_{\infty} = 10$, i.e., the offline distribution has a constant coverage. Then consider the Markovian policy class $\Pi: \Xcal \to \Delta(\Acal)$. Denote 
%     \begin{align*}
%         \tilde \pi = \argmin{\pi \in \Pi} \nbr{d^\pi - \mu}_{TV}.
%     \end{align*}
%     We have
%     \begin{align*}
%         \nbr{\frac{\pi^\ast}{\tilde \pi}}_{\infty} = \infty,
%     \end{align*}
%     i.e., the policy that minimizes the TV distance towards the offline distribution does not cover some states from the optimal policy's trajectory.
% \end{proposition}
% The implication of the previous result is that, in the worst case if most rewards are assigned to the states that are not covered by the learned policy, then the learned policy will have a constant gap to optimal policy. In fact, although the above statement is about the induced state marginal distribution, in the proof we can see that the resulted policy might take distinct actions than the optimal policy, so such a statement on the action distribution also holds. 

% \begin{remark}
%     The previous two hardness results are hard in comparison to the reset model setting, where in the reset model settings both setup can be easily solved. We summarize the comparison in \pref{tab:comparison}. 
% \end{remark}
% \begin{remark}
%     %One might notice that the construction of hardness results does not use the reward information, but the presence of reward information is irrelevant in the sparse reward setting, so our hardness results still hold in the sparse reward setting for any algorithms that use the reward information. 
%     Note that our hardness results are not equivalent to an information-theoretical lower bound, which is an interesting open problem.
% \end{remark}


% \subsection{Performance guarantee of the forward algorithm}
% Now we analysis \pref{alg:fail}. We start with an assumption that is the relaxation of \pref{assum:admissibility}, and the relaxed assumption is the one that we actually use in the analysis. Note that in the construction of the previous hardness results, this relaxed assumption is still violated. 
% \begin{assumption}[Admissibility in IPM.]\label{assum:admissibility_ipm}
%     There exists a partial polcy $\pi_{1:H}$ such that $\IPM_\Gcal(\pi_{1:h}, \mu_h) = 0, \forall h$.
% \end{assumption}

% We also introduce the common Bellman Completeness assumption, which is also made in \citet{sun2019provably}:

% \begin{assumption}[Completeness]\label{assum:completeness}
%     For any $h \in [H]$, for any $g \in \Gcal_{h+1}$, there exists $f \in \Gcal_h$ such that $f = \Tcal_h g$, where $\Tcal_h$ is the Bellman operator with respect to the offline distribution at time $h$: $\Tcal_h g(s_h) = \EE_{a_h \sim \mu_h(s_h)}  \EE_{s_{h+1} \sim P_h(s_h,a_h)}[ g(s_{h+1})]$. That is,
%     \begin{align*}
%         \max_h \max_{g \in \Gcal_{h+1}} \min_{f \in \Gcal_h} \left\|f - \Tcal_h g\right\|_\infty = 0.
%     \end{align*} 
% \end{assumption}

% Note that the previous two assumptions can both hold approximately, and here we assume that they hold exactly for simplicity. Now we can state the performance guarantee of the forward algorithm. The result is characterized in the IPM between the learned policy and the offline distribution.
% \begin{theorem}[Guarantee of \pref{alg:fail}]\label{thm:fail}
%     Assume \pref{assum:admissibility_ipm} and \pref{assum:completeness} hold. Suppose $|\Dcal^{\textsf{on}}| = |\Dcal^{\textsf{on}}| = N$, then with probability $1-\delta$, the returned policy $\pif$ satisfies that, for any $h \in [H]$,
%     \begin{align*}
%         \IPM_{\Gcal_{h}}(\pif_{1:h}, \mu_{h}) \leq h\epsforward(\delta, N),
%     \end{align*}
%     where 
%     \begin{align*}
%         \epsforward(\delta, N) := 8\sqrt{\frac{2A\log(2|\Gcal_{h}||\Pi|/\delta)}{N}} + \frac{16A\log(2|\Gcal_{h}||\Pi|/\delta)}{N} + \sqrt{\frac{A^2}{T}}.
%     \end{align*}
% \end{theorem}
    


% \subsection{Performance guarantee of FOOBAR}
% Finally we can show the performance guarantee of \Foobar. Different from the analysis of the forward algorithm, whose result is independent of the quality of the offline dataset, we should not expect \Foobar{} if the offline dataset does not cover the optimal policy's trajectory. Thus we introduce the coverage assumption:
% \begin{assumption}\label{assum:coverage}
% $\ccov(\pi^\ast) < \infty$.
% \end{assumption}

% Now we are ready to present our main result:
% \begin{theorem}\label{thm:foobar}
%     Suppose \pref{assum:admissibility_ipm}, \pref{assum:completeness}, and \pref{assum:coverage} hold. Then with probability $1-\delta$, the returned policy $\pib_{1:H}$ from \pref{alg:foobar} with discriminator constructed from \pref{eq:discriminator}, $N^{\textsf{for}}$ offline and forward samples, and $N^{\textsf{back}}$ backward samples, satisfies that
%     \begin{align*}
%         V^{\ast} - V^{\pib_{1:H}} \leq \epsilon,
%     \end{align*}
%     when 
%     \begin{align*}
%         N^{\textsf{for}} = O\rbr{\frac{\ccov^2(\pi^\ast)H^4A\log(|\Fcal||\Pi|/\delta)}{\epsilon^2}},~~ N^{\textsf{back}} = O\rbr{\frac{\ccov^2(\pi^\ast)H^4A\log(|\Fcal|/\delta)}{\epsilon^2}}.
%     \end{align*}
% \end{theorem}

% A few remarks are in order:
% \begin{remark}
% We can see that the sample required for the forward algorithm and backward algorithm are only different by a factor of $\log(|\Pi|)$. Usually the size of the function class and policy class are in the same order, so the sample complexity of the forward and backward algorithm are in the same order, and thus our algorithm performs a reduction from the trace model setting to the reset model setting with a constant overhead.
% \end{remark}

% \begin{remark}
%     Note that our result does not depend on size of the state space, and recall in the hardness result we showed that a polynomial dependency on the state space size is inevitable without the admissibility assumption. In the tabular case, in the worst case, the log size of function class will still be bounded by $SA$, which the final bound will be worse than the tightest bound in the tabular case \citep{zhang2023settling}. However, our result is favorable in the more general cases. For example, we can replace our coverage term with the one in \citet{song2022hybrid} without the polynomial dependency of the bilinear dimension \citep{du2021bilinear}. Finally, we conjecture that the worse action dependence is fundamental in the observation only setting (comparing to regular hybrid RL setting).
% \end{remark}

% \yuda{Add stationary results.}

% \section{Experiment}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figs/lockdiag.pdf}
%     \hspace{2cm}
%     \includegraphics[width=0.22\textwidth]{figs/hammer.png}
%     \caption{The combination lock environment.}
%     \label{fig:envs}
% \end{figure}

% In the experiments, we attempt to analyze the following questions: 1. How does \Foobar{} compare to the canonical hybrid RL algorithms, i.e., what is the price for the missing information in the offline dataset? 2. How does the performance compare with \Psdp{} if a reset model is available? 3. How robust is \Foobar{} against inadmissibility in practice? 

% To answer these questions, we use two benchmarks: the combination lock environment \citep{misra2020kinematic} and the hammer task of the Adroit robotics environment from the d4rl benchmark \citep{fu2020d4rl}. The visualization can be found in \pref{fig:envs}. Both environments are challenging to solve: the comb-lock environment requires careful exploration and previous online RL algorithms require additional representation learning algorithms to solve it \cite{misra2020kinematic,zhang2022efficient} because of its high-dimensional observation space and the good and bad states are mostly indistinguishable in the usual metrics. The hammer task is a challenging task in the d4rl benchmark for its high-dimension state and action space and difficult success condition. We adopt the binary reward version which makes the task even more challenging. 

% \subsection{Comparing to hybrid RL}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{figs/foobar_exp.pdf}
%     \caption{Comparing with hyrbid RL.}
%     \label{fig:hyrl}
% \end{figure}

% using expert dataset is due to lack of function appromination for multimodal distribution.

% \newpage
% \bibliography{refs} 

% \newpage
% \appendix
% \section{Discussion on admissibility}

% We first summarize a comparison among hybrid RL, hybrid RL with observation alone, and reset model with observation alone in \fref{tab:comparison}.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{p{4cm}p{3cm}p{4cm}p{3.5cm}}
%     \toprule
%     \multicolumn{1}{c}{The offline data Collected by} & \multicolumn{1}{c}{$s,a,r,s'$}  & \multicolumn{1}{c}{State Only} & \multicolumn{1}{c}{Reset with state only} \\
%     \midrule
%     A single policy & Solvable \newline \citep{song2022hybrid} & Solvable [Current work] & Solvable \newline \citep{bagnell2003policy} \\
%     A mixture policy & Solvable \newline \citep{song2022hybrid} & Solvable [Current work] \newline (\pref{prop:mixture}) & Solvable \newline \citep{bagnell2003policy} \\
%     Inadmissible distribution & Solvable \newline \citep{song2022hybrid} &  Hardness separation from the reset setting [Current Work]
%     \newline (\pref{prop:hard_data}, \ref{prop:hard_tv}) & Solvable \newline \citep{bagnell2003policy} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Table of comparison}
%     \label{tab:comparison}
% \end{table}

% Here we show that why the admissibility assumption holds if the offline dataset is collected by a mixture of policies.
% \begin{proposition}\label{prop:mixture}
%     Suppose the offline dataset is collected by a mixture of policies $\pi^1, \dots, \pi^K$, then there exists a single stochastic policy $\pi$ such that $\pi \overset{d}{=} \mu$.
% \end{proposition}

% \begin{proposition} 
%     There exists MDPs $\Mcal$ with deterministic transition and offline datasets $\{\Dcal\}$, with arbitrary sample size $\abr{\Dcal} = N \geq 2$, collected from the inadmissible offline distribution $\mu$ with constant coverage: $\nbr{\frac{d^{\pi^\ast}}{\mu}}_{\infty} = 2$. Then for any algorithms $\textsf{Alg}$, denote the dataset collected by $\textsf{Alg}$ as $D_{\textsf{Alg}}$. Then unless $\abr{D_{\textsf{Alg}}} = \Omega(A^H)$, we have that
%     \begin{align*}
%         \min_{\Dcal} \abr{D_{\textsf{Alg}} - \Dcal}_1 \geq 2.
%     \end{align*}
%     However, there exists an algorithm $\textsf{Alg}^{\textsf{reset}}$ that uses the offline dataset $\Dcal$ and reset model $\Mcal^{\textsf{reset}}$ that returns optimal policy $\pi^\ast$ with sample complexity $O(A)$.
% \end{proposition}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figs/hard_data.pdf}
%     \caption{Construction for \pref{prop:hard_data}.}
%     \label{fig:hard_data}
% \end{figure}
% \begin{proof}
%     Consider a binary tree MDP $\Mcal$, with two actions and deterministic transitions. Now we construct the offline dataset $\Dcal$ as following: for each horizon $h$, the dataset $\Dcal_h$ contains one samples from the optimal path and one samples from the other half of the tree. Thus by construction the dataset satisfies the coverage assumption. On the non-optimal data, we select them in the following way: on each level $h \geq 4$, the non-optimal data $s^{\textsf{no}}_h$ is an arbitrary non-child node of the last horizon $s^{\textsf{no}}_{h-1}$. Thus we see the previous non-optimal states provide no information for the current horizon, and thus the problem of finding $s^{\textsf{no}}_{h-1}$ is equivalent to a random search. However, unless $s^{\textsf{no}}_{h}$ is added to the dataset, we will have  $\abr{D_{h} - \Dcal_h}_1 \geq 2$, and thus we complete the proof. We show an example of such construction in \pref{fig:hard_data}, where the orange states denote the non-optimal states covered by the offline dataset and the blue states denote the optimal states covered by the offline dataset.
% \end{proof}

% \begin{proposition}
%     There exists MDP $\Mcal$ and inadmissible offline distribution $\mu$, such that $\nbr{\frac{d^{\pi^\ast}}{\mu}}_{\infty} = 10$, i.e., the offline distribution has a constant coverage. Then consider the Markovian policy class $\Pi: \Xcal \to \Delta(\Acal)$. Denote 
%     \begin{align*}
%         \tilde \pi = \argmin{\pi \in \Pi} \nbr{d^\pi - \mu}_1.
%     \end{align*}
%     We have
%     \begin{align*}
%         \nbr{\frac{\pi^\ast}{\tilde \pi}}_{\infty} = \infty,
%     \end{align*}
%     i.e., the policy that minimizes the TV distance towards the offline distribution does not cover some state from the optimal policy's trajectory.
% \end{proposition}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/hard_tv.pdf}
%     \caption{Construction for \pref{prop:hard_tv}.}
%     \label{fig:hard_tv}
% \end{figure}
% \begin{proof}
%     Consider the following one-step transition: where we start from $s_0$, and action $a_1,a_2$, and next states $s_1,s_2, s_3$, We have the following transition: $P(\cdot \mid s_0, a_1) = [0.95, 0.05, 0]$ and $P(\cdot \mid s_0, a_2) = [0, 0.9, 0.1]$. Consider the inadmissible offline state distribution over $s_1,s_2,s_3: \mu = [0.85,0.05,0.1]$. We can verify that the coverage assumption holds. Also suppose $\pi^\ast(s_0) = a_2$. Then by some calculation we have $\tilde \pi(s_0) = a_1$, and thus we have $\nbr{\frac{\pi^\ast}{\tilde \pi}}_{\infty} = \infty$, i.e., $\tilde \pi$ does not visit $s_3$ but $\pi^\ast$ does. An illustration of the construction can be found in \pref{fig:hard_tv}.
% \end{proof}


% \section{Proof of foobar}

% \subsection{Proof of \pref{thm:fail}}
% For the proof, we define a shorthand notation for the IPM distance as follows:
% \begin{align*}
%     d_{\Gcal_{h}}(\pi \mid \rho_{h-1}, \mu_{h}) := \IPM_{\Gcal_{h}}(\rho \circ_h \pi, \mu_{h}).
% \end{align*}
% Then we have the following guarantee of the \pref{alg:minmax}:
% \begin{lemma}[Guarantee of \pref{alg:minmax} (Theorem 3.1 of \citet{sun2019provably})] \label{lem:minmax}
% Assume \pref{assum:admissibility_ipm} holds. Suppose that $\Gcal_{h}$ is the discriminator class, $\rho$ is the roll in distribution, and $\mu$ is the offline distribution. Let $|\Dcal^{\textsf{on}}| = |\Dcal^{\textsf{on}}| = N$, then with probability $1-\delta$, the returned policy $\pi$ satisfies:
% \begin{align*}
%     d_{\Gcal_{h}}(\pi \mid \rho_{h-1}, \mu_{h}) \leq \min_{\pi' \in \Pi}d_{\Gcal_{h}}(\pi' \mid \rho_{h-1}, \mu_{h}) + \epsforward(\delta, N),
% \end{align*} 
% where 
% \begin{align*}
%     \epsforward(\delta, N) = 8\sqrt{\frac{2A\log(2|\Gcal_{h}||\Pi|/\delta)}{N}} + \frac{16A\log(2|\Gcal_{h}||\Pi|/\delta)}{N} + \sqrt{\frac{A^2}{T}}.
% \end{align*}
% \end{lemma}
% The proof of \pref{lem:minmax} can be found in \citet{sun2019provably}.

% Now we can prove the guarantee of \pref{alg:fail} in IPM, which is the property required in proving the final result.

% \begin{theorem}[Guarantee of \pref{alg:fail}]
% Assume \pref{assum:completeness} and \pref{lem:minmax} hold. Suppose $|\Dcal^{\textsf{on}}| = |\Dcal^{\textsf{on}}| = N$, then with probability $11\delta$, the returned policy $\pif$ satisfies that, for any $h \in [H]$,
% \begin{align*}
%     \IPM_{\Gcal_{h}}(\pif_{1:h}, \mu_{h}) \leq h\epsforward(\delta, N).
% \end{align*}
% \end{theorem}
% \begin{proof}
%     We can prove by induction. Consider the $h$ timesteps, where we have 
%     \begin{align*}
%         \IPM_{\Gcal_{h-1}}(\pif_{1:h-1}, \mu_{h-1}) \leq (h-1)\epsforward(\delta, N).
%     \end{align*}
%     Let $\pi^\ast := \argmin_{\pi \in \Pi} d_{\Gcal_h}(\pi \mid \pif_{1:h-1}, \mu_h)$, we have:
%     \begin{align*}
%         \IPM_{\Gcal_{h}}(\pif_{1:h}, \mu_{h}) &\leq d_{\Gcal_h}(\pi^\ast \mid \pif_{1:h-1}, \mu_h) + \epsforward(\delta, N) \tag{\pref{lem:minmax}} 
%         \\&= \max_{g \in \Gcal_h}\abr{\EE_{s_{h} \sim \pi_{h-1}, a_{h} \sim \pi^\ast(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1}) - \EE_{s_{h} \sim \mu_{h}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1})} + \epsforward(\delta, N) 
%         \\&\leq \max_{g \in \Gcal_h}\abr{\EE_{s_{h} \sim \pi_{h-1}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1}) - \EE_{s_{h} \sim \mu_{h}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1})} + \epsforward(\delta, N).
%     \end{align*}
%     Now denote $g^\ast_{h} = \argmax_{g \in \Gcal_h}\abr{\EE_{s_{h} \sim \pi_{h-1}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1}) - \EE_{s_{h} \sim \mu_{h}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g(s_{h+1})}$, we denote 
%     \begin{align*}
%         g^\ast_{h-1} = \argmin_{g \in \Gcal_{h-1}} \nbr{g - \Tcal_{h-1} g^\ast_{h}}_\infty,
%     \end{align*}
%     then we have 
%     \begin{align*}
%         &\abr{\EE_{s_{h} \sim \pi_{h-1}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g^\ast_h(s_{h+1}) - \EE_{s_{h} \sim \mu_{h}, a_{h} \sim \mu(s_{h}), s_{h+1} \sim P_h(s_h,a_h)}g^\ast_h(s_{h+1})} \\\leq& \abr{\EE_{s_{h} \sim \pi_{h-1}}g^\ast_{h-1}(s_{h}) - \EE_{s_{h} \sim \mu_{h}}g^\ast_{h-1}(s_{h})} + \epsilon^{\mathbf{be}} \tag{\pref{assum:completeness}} \\
%         \leq& \IPM_{\Gcal_{h-1}}(\pif_{1:h-1}, \mu_{h-1}) + \epsilon^{\mathbf{be}}  \\
%         \leq& (h-1)\epsforward(\delta, N) + \epsilon^{\mathbf{be}}, \tag{Inductive hypothesis}
%     \end{align*}
%     and thus we complete the proof.
% \end{proof}

% \subsection{Proof of \pref{thm:foobar}.}
% \label{app:proof_foobar}

% Now we prove the guarantee of \pref{alg:foobar}. We start with the guarantee of the value function estimation in \pref{alg:psdp_trace}.
% \begin{lemma}
%     With Probability $1-\delta$, the returned function $f_h$ satisfies:
%     \begin{align*}
%         \EE_{s_h \sim \pif_{1:h-1}} \max_{a_h} \left[ \left(f_h(s_h,a_h) - Q^{\pib_{h+1:H}}(s_h,a_h)\right)^2 \right] \leq 
%         \frac{H^2 A \log(|\Fcal|/\delta)}{n} := \epsback(\delta, n)^2.
%     \end{align*}
% \end{lemma}

% Recall our construction of the discriminator class $\Gcal_h$:
% \begin{align*}
%     \Gcal_h = \cbr{\max_a \abr{f(\cdot,a) - f'(\cdot,a)} + \abr{f(\cdot,a^\ast) - f'(\cdot,a^\ast)} : f,f' \in \Fcal_h, a^\ast = \argmax_{a} f(\cdot, a)}.
% \end{align*}
% The reason of such construction will be clear in the proof of \pref{thm:foobar}. But we first show that the size the discriminator class is bounded by the size of the value function class so it is not big. We assume that the value function class is finite for simplicity, but the results can be easily extended to the infinite case.
% \begin{lemma}\label{lem:discriminator_size}
%     $|\Gcal_h| \leq |\Fcal_h|^2$.
% \end{lemma}

% Then we can show the performance guarantee of \pref{alg:foobar}:
% % \begin{theorem}
% %     With probability $1-\delta$, the returned policy $\pib_{1:H}, 
% %     \begin{align*}
% %         V^\ast(s_0) - V^{\pib_{1:H}}(s_0) \leq C(\pi^\ast) H \epsilon_{\mathrm{stat}}(\delta, n) + C(\pi^\ast)H  \cdot \max_h d_\Fcal(d^{\pif}_h || \mu_h).
% %     \end{align*}
% % \end{theorem} 

% \begin{proof}
%     By performance difference lemma \citep{kakade2002approximately}, we have that 
%     \begin{align*}
%         &~~~~V^\ast - V^{\pib_{1:H}} \\&= \sum_{h=1}^H \EE_{s_h,a_h \sim \pi^\ast} \left[  Q^{\pib_{h+1:H}}(s_{h},a_h) - Q^{\pib_{h+1:H}}(s_{h},\pib_h(s_{h}))  \right] \\
%         &\leq  \sum_{h=1}^H \EE_{s_h,a_h \sim \pi^\ast} \left[  \max_a Q^{\pib_{h+1:H}}(s_{h},a) - Q^{\pib_{h+1:H}}(s_{h},\pib_h(s_{h}))  \right] \\
%         &=  \sum_{h=1}^H \EE_{s_h \sim \pi^\ast} \left[  \max_a Q^{\pib_{h+1:H}}(s_{h},a) - \max_{a'}f_h(s_h,a') + \max_{a'}f_h(s_h,a') - Q^{\pib_{h+1:H}}(s_{h},\pib_h(s_{h}))  \right] \\
%         &\leq  \sum_{h=1}^H \EE_{s_h \sim \pi^\ast} \left[  \max_a \left|Q^{\pib_{h+1:H}}(s_{h},a) - f_h(s_h,a) \right|+ \left|f_h(s_h,\pib_h(s_{h})) - Q^{\pib_{h+1:H}}(s_{h},\pib_h(s_{h}))\right|  \right] \\
%         &\leq  C(\pi^\ast)\sum_{h=1}^H \EE_{s_h \sim \mu_h} \left[  \max_a \left|Q^{\pib_{h+1:H}}(s_{h},a) - f_h(s_h,a) \right|+ \left|f_h(s_h,\pib_h(s_{h-1})) - Q^{\pib_{h+1:H}}(s_{h-1},\pib_h(s_{h}))\right|  \right] \\
%         &\leq  C(\pi^\ast)\sum_{h=1}^H \EE_{s_h \sim d^{\pif}_h} \left[  \max_a \left|Q^{\pib_{h+1:H}}(s_{h},a) - f_h(s_h,a) \right|+ \left|f_h(s_h,\pib_h(s_{h})) - Q^{\pib_{h+1:H}}(s_{h},\pib_h(s_{h}))\right|  \right] + \IPM_{\Gcal_h}\Fcal(d^{\pif}_h || \mu_h) \tag{Construction of $\Gcal$} \\
%         &\leq  C(\pi^\ast)H \epsback(\delta, N^{\textsf{back}}) + C(\pi^\ast)H^2 \epsforward(\delta,  N^{\textsf{for}}). \\
%     \end{align*}
%     By plugging in the defintion of $\epsback$ and $\epsforward$, we have 
%     \begin{align*}
%         V^\ast - V^{\pib_{1:H}} \leq O\rbr{C(\pi^\ast) H \sqrt{\frac{H^2A\log(|\Fcal|/\delta)}{N^{\textsf{back}}}} + C(\pi^\ast) H \sqrt{\frac{A\log(|\Fcal||\Pi|/\delta)}{N^{\textsf{for}}}} },
%     \end{align*}
%     by setting $T = AN^{\textsf{for}}$ and by \pref{lem:discriminator_size}, finally by setting $N$ properly, we have the desired result.
% \end{proof}

% \section{Experiment Details}\label{app:exp} 

% \subsection{Combination Lock Environment}
% In our experiment, the \textit{diabolical combination lock} problem (referenced as comb-lock) served as the testing ground for our algorithm. This scenario is defined by a horizon of length $H$ and involves a selection from 10 distinct actions. At each point in the sequence, denoted as step $h$, the system can be in one of three potential hidden states, symbolized as $z_{i;h}$ for $i$ values in the set ${0,1,2}$. States $z_{i;h}$, where $i$ falls within ${0,1}$, are considered advantageous, while the state $z_{2;h}$ is categorized as disadvantageous.

% For each advantageous state $z_{i;h}$ (where $i$ is either 0 or 1), an action, denoted as $a_{i;h}$, is chosen randomly from the pool of 10 actions. In such states, executing the action $a_{i;h}$ leads to a transition to either state $z_{0;h+1}$ or $z_{1;h+1}$, with each possibility having an equal chance of occurrence. Choosing any action other than $a^\ast_{i;h}$ in these states ensures a move to the state $z_{2;h+1}$. In the state $z_{2;h}$, the agent's action choice does not affect its transition, which is always to $z_{2;h+1}$.

% The reward structure is such that a reward of 1 is assigned at state $z_{i;H}$ for $i \in {0,1}$. There is also a 50\% probability of receiving a minor, inverted reward of 0.1 when transitioning from a favorable to an unfavorable state. All other state transitions or states do not yield any reward.

% Observations in this problem, denoted as $s$, have a dimensionality of $2^{\lceil{\log(H+4)}\rceil}$. This is formulated by concatenating the one-hot vectors representing the hidden state $z$ and the horizon $h$, to which noise from the distribution $\Ncal(0,0.1)$ is added for each dimension. This is then adjusted with zeroes where necessary and processed through a Hadamard matrix. The starting state distribution is uniformly divided among $z_{i;0}$ for $i \in {0,1}$. An important aspect to note is that the ideal strategy involves consistently selecting the action $a^*_{i;h}$ at each step $h$. Once the agent enters a disadvantageous state, it remains in such states till the episode concludes, thus forfeiting the opportunity for a significant end reward. This presents a significant challenge in terms of exploration, as a strategy based on random uniform selection yields only a $10^{-H}$ chance of reaching the intended goals.

% \end{document}

